Shape Matters: Understanding the Implicit Bias of the Noise Covariance

The noise in stochastic gradient descent (SGD) provides a crucial implicit regularization effect for training overparameterized models. Prior theoretical work largely focuses on spherical Gaussian noise, whereas empirical studies demonstrate the phenomenon that parameter-dependent noise -- induced by mini-batches or label perturbation -- is far more effective than Gaussian noise. This paper theoretically characterizes this phenomenon on a quadratically-parameterized model introduced by Vaskevicius et el. and Woodworth et el. We show that in an over-parameterized setting, SGD with label noise recovers the sparse ground-truth with an arbitrary initialization, whereas SGD with Gaussian noise or gradient descent overfits to dense solutions with large norms. Our analysis reveals that parameter-dependent noise introduces a bias towards local minima with smaller noise variance, whereas spherical Gaussian noise does not. Code for our project is publicly available.

==> warmup.tex <==
\section{Warming-up with Illustrating Examples\tnote{Warming up? @colin/jason :)}}
In this section, we use toy examples to illustrate two different implicit biases of noises, one weak bias that could come from parameter-independent noise and one stronger bias that comes from parameter-dependent noise.

\subsection{Analyzing the Implicit Bias of Noises via  Potential Functions}\label{subsec:effect1}

Although there are strong empirical evidence~\citep{keskar2016large} and theoretical intuition on the implicit bias of SGD towards flat local minima, we lack mathematical tools to analyze the behavior of stochastic updates. Though the Langevin dynamics converges to the Gibbs distribution which has a beautiful analytical form, solving the stationary distribution of a general stochastic process is likely intractable~\citep{?}. 

In this paper, we propose to use carefully constructed potential functions to characterize the behavior of noises. In this subsection, we demonstrate the power of a potential function on a proof-of-concept toy loss function. 
\newcommand{\R}{\mathbb{R}}
In this subsection, let the loss function be $\ell(v) \triangleq \norm{v}^2_2 (v^\top x)^2$ where $x\in \R^2$ is a given unit vector and $v\in \R^2$ is the parameter variable.  The potential function is visualized in Figure~\ref{?}. Let $x^\perp$ be the unit vector orthogonal to $x$. We observe that the set of global minima forms the line $\{v : v = \alpha x^\perp\}$. Moreover, $v=0$ is the flattest global minimum whereas the curvature becomes sharper as we move towards infinity along the line of global minima.




However, let's think of the situation when we add gaussian noise to the gradient in the direction of $x$, i.e., adding $\xi x$ to gradient where $\xi\sim \mathcal{N}(0, 1)$. 
Since this only changes $v_x$ but not $v_{x^\perp}$, this may not be obviously doing anything useful. But as we will show below, this actually brings the iterate away from ``sharp'' local minima and drives $v_{x^{\perp}}$ to decrease to $0$, where this function is the most ``flat''. \cnote{I'm slightly confused by the wording here because at first you say it doesn't change $v_{x^{\perp}}$, and next you say it drives it to 0}

Actually we can show this effect via a simple potential function $\norm{v_{x^\perp}}^2$. Since adding the noise only changes $v_{x}$, it might seem like adding noise or not doesn't influence $\norm{v_{x^\perp}}^2$. However, if we look at the inner product of gradient and of this potential function, we see $\langle \nabla \ell(v), \nabla\norm{v_{x^\perp}}^2\rangle = 2(v^\top x)^2 \norm{v_{x^\perp}}^2 \ge 0\rangle$, so the gradient term always decreases this potential function. \cnote{I think this could be explained better. At first I read gradient term always decreases potential function, and I wondered why we needed the noise. It was only after I realized that we can't have $(v^\top x)^2$ be zero that I understood why we need the noise} Notice that without noise $v^\top x$ can become $0$ very quickly (i.e, converge), but noise keeps it positive so decreases this potential in a ``second order'' manner. Figure~\ref{fig:illustrate} gives a graphic illustration of this effect.

Although this example captures some effect people observe in real world models (e.g., bias toward flat minimum), one may hope that any noise should have the effect mentioned here, since its effect is simply keeping the loss not to be too small. Actually this example ignores the noise structure that could occur in real-world models, especially its dependency on parameter which is empirically observed to be crucial. \jeff{add more relation to our 2-layer model as in the doc?}














